Combination of Domain Knowledge and Deep Learning for Sentiment Analysis of Short and Informal Messages on Social Media

Sentiment analysis has been emerging recently as one of the major natural language processing (NLP) tasks in many applications. Especially, as social media channels (e.g. social networks or forums) have become significant sources for brands to observe user opinions about their products, this task is thus increasingly crucial. However, when applied with real data obtained from social media, we notice that there is a high volume of short and informal messages posted by users on those channels. This kind of data makes the existing works suffer from many difficulties to handle, especially ones using deep learning approaches. In this paper, we propose an approach to handle this problem. This work is extended from our previous work, in which we proposed to combine the typical deep learning technique of Convolutional Neural Networks with domain knowledge. The combination is used for acquiring additional training data augmentation and a more reasonable loss function. In this work, we further improve our architecture by various substantial enhancements, including negation-based data augmentation, transfer learning for word embeddings, the combination of word-level embeddings and character-level embeddings, and using multitask learning technique for attaching domain knowledge rules in the learning process. Those enhancements, specifically aiming to handle short and informal messages, help us to enjoy significant improvement in performance once experimenting on real datasets.

==> authors_bio.tex <==
\section*{Biographical notes}
\paragraph*{Khuong Vo} received his B.Eng. (Honors) degree in Computer Science from Ho Chi Minh City University of Technology in 2017. His current research focuses on applying machine learning and deep learning to solve real-world problems, especially in social media and e-commerce fields.
\paragraph*{Tri Nguyen} received his B.Eng. (Honors) degree in Computer Science from Ho Chi Minh City University of Technology in 2017. His current research interests include natural language processing, image processing and deep learning.
\paragraph*{Dang Pham} received his B.Sc degree in Computer Science from Ho Chi Minh University of Science in 2014. Currently, he is pursuing a Master degree in the same university. His research interests include image processing, natural language processing and neuroscience.
\paragraph*{Mao Nguyen} received his B.Sc degree in Computer Science from Ho Chi Minh University of Science in 2011 and holds a Master degree in Computer Science from John von Neumann Institute in 2015. His current research interests include data mining/machine learning, computer vision and statistical inference methods.
\paragraph*{Minh Truong} received his B.Eng. degree in Computer Science from Ho Chi Minh City University of Technology in 2012. He won VEF fellowship in 2014 to study at Iowa State University, USA, and completed his Master degree in 2016 under the supervision of Prof. Srikanta Tirthapura. His primary focuses now are on natural language processing and large-scale distributed system based on Hadoop.
\paragraph*{Trung Mai} is currently working as a researcher in the Faculty of Computer Science and Engineering, Ho Chi Minh City University of Technology. He received his M.Eng (2015) in Computer Science from James Cook University, Australia and B.Eng (2013) in Computer Engineering from Auckland University of Technology, New Zealand. His current research interests involve machine learning and deep learning.
\paragraph*{Tho Quan} is an Associate Professor in the Faculty of Computer Science and Engineering, Ho Chi Minh City University of Technology (HCMUT), Vietnam. He received his B.Eng. degree in Information Technology from HCMUT in 1998 and received Ph.D degree in 2006 from Nanyang Technological University, Singapore. His current research interests include formal methods, program analysis/verification, the Semantic Web, machine learning/data mining and intelligent systems. Currently, he heads the Department of Software Engineering of the Faculty. He is also serving as the Chair of Computer Science Program (undergraduate level).
